Integrating Physiological Time Series and Clinical Notes with Deep Learning for Improved ICU Mortality Prediction

Intensive Care Unit Electronic Health Records (ICU EHRs) store multimodal data about patients including clinical notes, sparse and irregularly sampled physiological time series, lab results, and more. To date, most methods designed to learn predictive models from ICU EHR data have focused on a single modality. In this paper, we leverage the recently proposed interpolation-prediction deep learning architecture(Shukla and Marlin 2019) as a basis for exploring how physiological time series data and clinical notes can be integrated into a unified mortality prediction model. We study both early and late fusion approaches and demonstrate how the relative predictive value of clinical text and physiological data change over time. Our results show that a late fusion approach can provide a statistically significant improvement in mortality prediction performance over using individual modalities in isolation.

==> old_exps.tex <==
%!TEX root = amia.tex

\section{Experiments and Results}

In this section, we present experiments\footnote{We plan to share all data processing and model learning code on Github.} and results. Our experiments focus on the relative predictive performance of text-only models, time series-only models, and fusion models for the problem of in-hospital mortality prediction. The prediction output is a single binary variable representing the occurrence of in-hospital morality more than 48 hours after admission.
The time series inputs to the prediction task are sparse and irregularly sampled physiological time series. We consider making predictions using physiological time series data available between 6 and 48 hours after admission. The text inputs to the prediction task consists of text content known at the time of admission and progress notes that vary through time.  
% also vary through time and include text content known at the time of admission, text content known up to and including the first 24 hours after admission, and text content known up to and including the first 48 hours after admission. 
We begin by briefly describing the data set used, followed by the set of baseline and comparison models,  the empirical protocols used, and finally the results. 

\begin{table}[h]
\centering
\caption{Features extracted from MIMIC III}
\label{table:mis}
           \footnotesize
            %\begin{minipage}{.5\linewidth}
                \begin{tabular}[h]{l c}
                
                 \toprule
                 {feature} & {Sampling Rate}\\
                    \midrule
                    SpO2 &  $0.80$\\
                    HR  &  $0.90$\\
                    RR &  $0.48$\\
                    SBP &  $0.59$\\
                    DBP &  $0.60$\\
                    Temp &  $0.19$\\
  
                    \bottomrule
                    \end{tabular}  
                    \,\,\,\,\,\,
                   % \end{minipage} &
       %\begin{minipage}{.5\linewidth}
                \begin{tabular}[h]{l c}
                 \toprule
                 {feature}  & {Sampling Rate}\\
                    \midrule
                    TGCS &  $0.14$\\
                    CRR & $0.06$\\
                    UO & $0.20$\\
                    FiO2 &$0.06$\\
                    Glucose &$0.10$\\
                    pH &$0.04$\\
                    \bottomrule
                    \end{tabular}
                   % \end{minipage}
                \end{table}

\subsection{Dataset}
Our experiments are based on the publicly available MIMIC-III dataset \citep{johnson2016mimic}. This data set contains sparse and irregularly sampled physiological signals, discharge summaries, progress notes, medications, diagnostic codes, in-hospital mortality, length of stay, demographics information and more. It consists of approximately 58,000 hospital admission records. We focus on predicting in-hospital mortality using both the clinical text and time series data. We use 42,984
records for our experiments obtained after removing newborns and hospital admission records containing no discharge summaries  or with length of stay less than 48 hours. We extract 12 standard physiological variables from each of the records.  Table \ref{table:mis} shows the variables and sampling rates (per hour). We use text data known at the time of admission such as chief complaints, past medical history and history of present illness. We take care in extracting this information from discharge summaries in order to avoid any information leak. We also extract progress notes from non-discharge reports such as respiratory, ECG, echo, radiology, and nursing reports. We use the date and time stamps on these reports to create a set of notes available up to the first $n$ hours after admission. 

%For some experiments, we use all notes available up to and including the first 24 hours after admission, as well as all notes available up to and including the first 48 hours after admission.

%\subsection{Prediction Task}
%In our experiments, each admission record corresponds to one data case $(\mbf{s_n},\mbf{v_n}, y_n)$. 
%Each data case $n$ consists of a sparse and irregularly sampled time series $\mbf{s}_n$ with $D=12$ 
%dimensions, and unstructured clinical text data $\mbf{v}_n$.  Each dimension $d$ 
%of $\mbf{s}_n$ corresponds to one of the $12$ vital sign time series mentioned in Table \ref{table:mis}. 
%$y_n$ is a binary indicator where $y_n=1$ indicates that the patient died at any point within the hospital 
%stay following the first 48 hours and $y_n=0$ indicates that the patient was discharged at any point after
% the first 48 hours. There are 3,623(8.43\%) patients with a $y_n=1$ mortality label. 
% The complete data set is $\mathcal{D}=\{(\mbf{s_n},\mbf{v_n},y_n)|n=1,...,N\}$, and there
%are $N=42,984$ data cases. The goal in the classification task is to learn a function $h$ of the
%form $\hat{y}_n \leftarrow h(\mbf{s}_n,\mbf{b}_n)$ where $\hat{y}_n$ is a discrete value.

\subsection{Baseline Models}
We compare fusion models with a number of baseline approaches that model the physiological 
time series or the clinical text data individually.  \citet{shukla2019interpolationprediction} show that the 
interpolation-prediction network outperforms 
a range of baseline and recently proposed models on both classification and regression tasks for 
sparse and irregularly sampled time series. Hence, we use interpolation-prediction network as our 
time series-only baseline model. We use the pre-trained text-only models described in Section \ref{sec:text} to provide text-only baselines.


\subsection{Empirical Protocols}
We divide the dataset into standard train (60\%), validation (20\%) and test (20\%) sets. All models are trained to minimize the cross entropy loss. For all of the models, we independently tune the hyper-parameters 
such as number of hidden layers and hidden units on the validation set. The neural network models are learned using the Adam optimizer. 
Early stopping is used on the validation set. The final outputs of the hidden layers are used in a logistic layer that predicts the class. We evaluate all the 
models using an estimate of generalization performance computed on test set. 
We report the performance on the test set in terms of the average area under the ROC
curve (AUC score).

\subsection{Results}
In this section, we present the results of the mortality prediction 
experiments. We begin with text-only and time series-only baseline results, followed by fusion model results.

%  \midrule
%  {USE} / RNN   & 0 & $0.8027$\\ 
%  WSE / RNN     & 0 & $0.7800$\\
%  WE / CNN      & 0 & $0.7589$\\
%  TF-IDF / 1-NN & 0 & $0.8153$\\
%  TF-IDF / 1-NN & 24 & $0.8410$\\
%  TF-IDF / 1-NN & 48 & $0.8627$\\

\begin{table*}
\centering
\begin{minipage}{.4\textwidth}
%\centering
\caption{Text-Only}
%\footnotesize
\begin{tabular}{ l c c c} 
 \toprule
{\bf Text Model} & {\bf Hours from}& {\bf AUC}   \\
& {\bf Admission} &\\
 \midrule
 {USE} / RNN   & 0 & $0.7473$\\ 
 WSE / RNN     & 0 & $0.7364$\\
 WE / CNN      & 0 & $0.7589$\\
 TF-IDF / 1-NN & 0 & $0.7965$\\
 TF-IDF / 1-NN & 24 & $0.8410$\\
 TF-IDF / 1-NN & 48 & $0.8627$\\
\bottomrule
 \end{tabular}
 \label{table:text}
\end{minipage}
%
\begin{minipage}{.28\textwidth}
\centering
\caption{Time Series-Only}
%\footnotesize
\begin{tabular}{ c c c} 
 \toprule
 {\bf Hours from} & {\bf AUC }    \\
 {\bf Admission} \\
 \midrule
$	6	$	&	$	0.7106	$	\\
$	12	$	&	$	0.7380	$	\\
$	18	$	&	$	0.7645	$	\\
$	24	$	&	$	0.7759	$	\\
$	36	$	&	$	0.7958	$	\\
$	48	$	&	$	0.8245	$	\\
\bottomrule
 \end{tabular}
 \label{table:vitals}
 \end{minipage}%
%
 \begin{minipage}{.3\textwidth}
 \caption{Fusion }
% \centering
 \begin{tabular}{ c c c  c c } 
  \toprule
  {\bf Hours from } & {\bf Early}  &  {\bf Late} \\
  {\bf Admission} &  {\bf AUC }  & {\bf AUC }  \\
  \midrule
 $	6	$&$	0.785	$&$	0.8027	$\\
 $	12	$&$	0.7916	$&$	0.8161	$\\
 $	18	$&$	0.8046	$&$	0.8138	$\\
 $	24	$&$	0.8126	$&$	0.8256	$\\
% $	30	$&$	0.8284	$&$	0.8324	$\\
 $	36	$&$	0.8291	$&$	0.832	$\\
% $	42	$&$	0.838	$&$	0.8376	$\\
 $	48	$&$	0.8427	$&$	0.8453	$\\
 \bottomrule
  \end{tabular}
 \label{table:text_vitals}
\end{minipage}
\end{table*}

\begin{figure*}[t]
\hfill
\begin{minipage}{0.47\textwidth}
\centering
\includegraphics[width=0.98\linewidth]{Figures/comparisons.pdf}
\caption{Performance comparison on the mortality prediction task with
text available at admission only.}
\label{fig:comp-admit}
\end{minipage}
\hfill
\begin{minipage}{0.47\textwidth}
\centering
%\includegraphics[width=0.98\linewidth]{Figures/compare5.pdf}
\includegraphics[width=0.98\linewidth]{Figures/comparisons2.pdf}
\caption{Performance comparison on the mortality prediction task with
text available at admission, 24 and 48 hours.}
\label{fig:comp-rolling}
\end{minipage}
\hfill
\end{figure*}


\textbf{Text-Only Baselines:} Table \ref{table:text} shows the classification performance for the text-only models described in Section \ref{sec:text}. We evaluate all models in the case of text data available at the time of admission. These results show that the TF-IDF-based model performs slightly better than the embedding methods. This may be due to the fact that health-specific concepts are not well represented in the standard Glove embeddings used. Another possible reason could 
be the use of abbreviated terms, which are quite common in clinical notes. For this reason, we only consider the TF-IDF model when making predictions based on all notes available within the first 24 and 48 hours. We can see that prediction performance using the TF-IDF model increases significantly as more text data become available over time. 

\textbf{Time Series-Only Baseline:} Table \ref{table:vitals} assesses 
the predictive performance of the time series-only interpolation-prediction network described in Section \ref{sec:interp}. As expected, predictive performance  increases as the amount of observed physiological data increases. Comparing to the results in Table \ref{table:text}, we can see that the predictive value of the clinical text available at the time of admission exceeds that of the available physiological data until near the end of the 48 hour period following admission. The next set of experiment aims to assess whether these two modalities can result in improved performance when fused.

\textbf{Fusion Approaches:} Based on the observed success of the TF-IDF-based model in the text-only baseline experiments, we examine the performance of fusion approaches using the TF-IDF-based model to embed the clinical text data. We begin by assessing the performance of a fusion approach that only has access to the clinical text data available at the time of admission, but increasing amounts of physiological time series data up to the end of the 48 hour period following admission. 
Table \ref{table:text_vitals} shows the classification performance of the early and late fusion models under this experimental scenario. Figure \ref{fig:comp-admit} shows the performance of early and late fusion relative to the time series-only and text-only baselines. We can see that the late fusion approach achieves better results than the early fusion approach, while both significantly improve on the time series-only baseline. However, we see that all three models that incorporate physiological data increase in predictive performance as the amount of physiological data increases. Further, we see that the performance gap between fusion and time series-only models decreases over time, which indicates that the advantage provided by the initial fusion with text data available at time of admission decreases over time as that information becomes less relevant. Finally, we note that the fusion models initially exhibit lower performance than the text-only TF-IDF baseline, but go on to match and then out-perform the text-only baseline.

Next, we consider the fusion process as increasing volumes of text data become available through time, as well as increasing volumes of physiological data. For this experiment, we consider only the TF-IDF-based text embedding model and limit the discussion to the late fusion approach as these models have achieved the best performance in our experiments to date. We consider incorporating text data known at admission at time 0, followed by the text of all  notes known up to the end of the first 24 hours following admission, and the text of all  notes up to the first 48 hours following admission. The results of this experiment are shown in Figure \ref{fig:comp-rolling}. We can see that there is a significant performance jump by incorporating notes available up to 24 hours, and a much smaller jump when incorporating notes available through the end of the full 48 hour period. We can also see that the performance of the fused model always exceeds that of the corresponding text-only baseline active at a given point in time, with performance generally rising as additional physiological data become available. By comparing with Figure \ref{fig:comp-admit}, we can see that the addition of text data at 24 and 48 hours past admission results in a final fused model that significantly outperforms models that only have access to text data from the time of admission.




%\begin{table}[h]
%\caption{Classification performance with joint modeling of physiological time series and clinical text data}
%\begin{center}
%\begin{tabular}{ c c c  c c } 
% \toprule
% {\bf Hours from } & \multicolumn{2}{c}{\bf Early Fusion}  &  \multicolumn{2}{c}{\bf Late Fusion } \\
% {\bf Admission} &  {\bf AUC } & {\bf AUPRC } & {\bf AUC } & {\bf AUPRC } \\
% \midrule
%$	6	$&$	0.785	$&$ 0.2735 $&$	0.8027	$&$	0.3048 $\\
%$	12	$&$	0.7916	$&$ 0.2942 $&$	0.8161	$&$	0.3252$\\
%$	18	$&$	0.8046	$&$ 0.3008 $&$	0.8138	$&$	0.3317$\\
%$	24	$&$	0.8126	$&$ 0.3129 $&$	0.8256	$&$	0.3489$\\
%$	30	$&$	0.8284	$&$ 0.3523 $&$	0.8324	$&$	0.3654$\\
%$	36	$&$	0.8291	$&$ 0.3298 $&$	0.832	$&$	0.3710$\\
%$	42	$&$	0.838	$&$ 0.3851 $&$	0.8376	$&$	0.3815$\\
%$	48	$&$	0.8427	$&$ 0.4074 $&$	0.8453	$&$	0.4176$\\
%\bottomrule
% \end{tabular}
%\end{center}
%\label{table:text_vitals}
%\end{table} 
%
%\begin{figure}[h]
%\centering
%\includegraphics[width=0.6\linewidth]{Figures/compare4.pdf}
%\caption{Performance comparison on mortality prediction task}
%\label{fig:comp}
%\end{figure}

%\vspace{5mm}







